UniVS: Unified and Universal Video Segmentation with Prompts as Queries

Despite the recent advances in unified image segmentation (IS), developing a unified video segmentation (VS) model remains a challenge. This is mainly because generic category-specified VS tasks need to detect all objects and track them across consecutive frames, while prompt-guided VS tasks require re-identifying the target with visual/text prompts throughout the entire video, making it hard to handle the different tasks with the same architecture. We make an attempt to address these issues and present a novel unified VS architecture, namely UniVS, by using prompts as queries. UniVS averages the prompt features of the target from previous frames as its initial query to explicitly decode masks, and introduces a target-wise prompt cross-attention layer in the mask decoder to integrate prompt features in the memory pool. By taking the predicted masks of entities from previous frames as their visual prompts, UniVS converts different VS tasks into prompt-guided target segmentation, eliminating the heuristic inter-frame matching process. Our framework not only unifies the different VS tasks but also naturally achieves universal training and testing, ensuring robust performance across different scenarios. UniVS shows a commendable balance between performance and universality on 10 challenging VS benchmarks, covering video instance, semantic, panoptic, object, and referring segmentation tasks. Code can be found at \url{https://github.com/MinghanLi/UniVS}.

==> figs/contrastive_learning.tex <==
\begin{figure}[t]
    \vspace{+1mm}
     \centering
     \includegraphics[width=0.95\linewidth]{figs/fig/contrastive_learning.jpg}
     \vspace{-1mm}
     \caption{Illustration of contrastive learning for ReID loss.}\label{fig:ctt_loss}
     \vspace{-4mm}
\end{figure}

==> figs/maskdec_arch_sub.tex <==
\begin{figure}[t]
     \vspace{-1mm}
     \centering
     \includegraphics[width=1.03\linewidth]{figs/fig/mask_dec_arch_prompt.jpg}
     \vspace{-7mm}
     \caption{
     Mask decoder architectures of (a) SEEM \cite{seem}, (b) UNINEXT \cite{uninext} and (c) our UniVS, which differ in image and prompt interaction. Feed-forward network (FFN) is omitted here. 
     }\label{fig:maskdec_sub}
     \vspace{-4mm}
\end{figure}

==> figs/vs_tasks.tex <==
\begin{figure*}[!h]
     \vspace{-1mm}
     \centering
     \includegraphics[width=0.98\linewidth]{figs/fig/vs_tasks.png}
     \vspace{-1mm}
     \caption{Illustration of different video segmentation (VS) tasks.  Category-specified VS includes VIS, VSS and VPS tasks, while prompt-specified VS consists of VOS, RefVOS and PVOS tasks. }\label{fig:vs_tasks}
     \vspace{-4mm}
\end{figure*}

==> figs/vs_tasks_0e48.tex <==
\begin{figure}[t]
     \vspace{-1mm}
     \centering
     \includegraphics[width=0.999\linewidth]{figs/fig/visualization/yt21_0e487d0704.png}
     \vspace{-6mm}
     \caption{Visualization examples of UniVS on different VS tasks. 
     The entity categories of VIS and VSS/VPS are from YT21 and VIPSeg datasets, respectively.
     }\label{fig:vs_tasks_0e48}
     \vspace{-1mm}
\end{figure}

==> tables/abl_maskdec_img.tex <==
\begin{table*}[!t]
\centering
{\small 
\begin{tabular}{p{0.12\linewidth}|p{0.03\linewidth}<{\centering}p{0.025\linewidth}<{\centering}p{0.03\linewidth}<{\centering}|p{0.032\linewidth}<{\centering}p{0.037\linewidth}<{\centering}|p{0.032\linewidth}<{\centering}p{0.032\linewidth}<{\centering}|p{0.035\linewidth}<{\centering}p{0.035\linewidth}<{\centering}|p{0.027\linewidth}<{\centering}p{0.027\linewidth}<{\centering}|p{0.025\linewidth}<{\centering}p{0.037\linewidth}<{\centering}|p{0.05\linewidth}<{\centering}}
\Xhline{0.8pt}
\rowcolor{LightCyan}
\multicolumn{1}{l|}{Training stages} & \multicolumn{5}{c|}{\textbf{Stage 1}} & \multicolumn{9}{c}{\textbf{Satge 2}} \\
\rowcolor{LightCyan}
\multicolumn{1}{l|}{Training datasets} & \multicolumn{5}{c|}{COCO + SA1B(2.5\%)} & \multicolumn{9}{c}{+YTVIS21+OVIS+VIPSeg+RefYT} \\
\hline
\hline
\rowcolor{LightCyan}
Tasks & PS & IS & SS & \multicolumn{2}{c|}{VOS} & \multicolumn{2}{c|}{VIS} &  \multicolumn{2}{c|}{VSS} &  \multicolumn{2}{c|}{VPS} & \multicolumn{2}{c|}{VOS} & \multicolumn{1}{c}{RefVOS}  \\
\hline
 Inf. datasets & \multicolumn{3}{c|}{\small COCO}  &{\small \!YT18\ }  & {\small \!\!MOSE } & {\small YT21}  & {\small OVIS} & \multicolumn{2}{c|}{\small VSPW} & \multicolumn{2}{c|}{\small VIPSeg} &{\small \!\!YT18\ }  & {\small \!\!MOSE } & RefYT \ \\
  Metrics & PQ & \!mAP & \!mIoU & G & G & mAP & mAP & mIoU & \!\!mVC$_8$ & VPQ & STQ & G & G & J\&F\\
\hline
\multicolumn{10}{l}{\it training on individual tasks (without SA1B)} \\
Ind. SOTA  &  51.9 & 41.7 & 61.7 &  &  & 48.3 & 34.0 & 42.3 & 86.8 & 43.2 & 43.1 & 87.0 & 61.2 & 61.2 \\
\hline 
\hline
M2F         & 47.3 & 40.0 & 57.4 & 57.4 &  & 45.9 & 17.2 & & & 40.1 & 37.9 & \\  % 38.1(yt21) & 28.6(ovis)
SEEM        & 47.7 & 41.3 & 59.4 & 62.1 &  & 49.2 & 14.7 & & & 39.3 & 34.2 & \\
d           & 47.8 & 41.4 & 59.8 & 57.4 &  & 51.4 & 15.0 & & & 42.0 & 38.1 & \\
d+l2p       &      &      &      &      &  &      & 21.0 & & &  &  \\
d+l2p+long  &      &      &      &      &  &      &      & & &  &  \\
% b
% d-p2l & 45.2 & 39.9 & 55.1 & &  \\
\Xhline{0.8pt}
\end{tabular}
}
\vspace{-1mm}
\caption{\small Ablation studies on various architectures of mask decoder. In the models with open-voc ability, the classification loss needs to replace the original BCE loss (Softmax) with multi-class focal loss (Sigmoid). All models are trained on same settings and datasets of the first two training stages.
} \label{tab:abl_maskdec}
\vspace{-1mm}
\end{table*}

==> tables/abl_prompt_attn.tex <==
\begin{table*}[!t]
\centering
{\footnotesize 
\begin{tabular}{p{0.04\linewidth}<{\centering}p{0.04\linewidth}<{\centering}|p{0.025\linewidth}<{\centering}p{0.03\linewidth}<{\centering}|p{0.025\linewidth}<{\centering}p{0.025\linewidth}<{\centering}|p{0.035\linewidth}<{\centering}|p{0.05\linewidth}<{\centering}}
\Xhline{0.8pt}
\rowcolor{LightCyan}
\multicolumn{2}{c|}{Tasks} & \multicolumn{2}{c|}{VIS} &  \multicolumn{2}{c|}{VPS} & \multicolumn{1}{c|}{VOS} & RefVOS \\
\hline
\multirow{2}{*}{P$\rightarrow$Q} & \multirow{2}{*}{PCA}  & { YT21}  & {OVIS} & \multicolumn{2}{c|}{ VIPSeg} &{ YT18\ }  & RefYT \ \\
       & & mAP & mAP & VPQ & STQ & G  & J\&F\\
\hline
\crossmark   & \crossmark   & 45.9 & 17.2 & 40.1 & 37.9 & 56.3  \\
$\checkmark$ & \crossmark   & 39.9 & 10.0 & 40.6 & 37.3 & 58.6 \\ % learn for VPS
$\checkmark$ & $\checkmark$ & 52.7 & 21.7 & 38.6 & 45.8 & \\
\Xhline{0.8pt}
\end{tabular}
}
\vspace{-2mm}
\caption{\small Ablation studies on prompt as queries (P$\rightarrow$Q) and the number layers of prompt cross-attention (PCA). Mean prompt queries only cannot perceive the granularity of the targeted object. For instance, `a person' or `a T-shirt'.
} \label{tab:abl_details}
\vspace{-2mm}
\end{table*}

==> tables/abl_tracker.tex <==
\begin{table}[!t]
\centering
{\footnotesize
\begin{tabular}{p{0.045\linewidth}<{\centering}p{0.12\linewidth}<{\centering}|p{0.05\linewidth}<{\centering}p{0.065\linewidth}<{\centering}|p{0.045\linewidth}<{\centering}p{0.06\linewidth}<{\centering}|p{0.075\linewidth}<{\centering}|p{0.105\linewidth}<{\centering}}
\Xhline{0.8pt}
\rowcolor{LightCyan}
\multicolumn{2}{c|}{Video Tasks} & \multicolumn{2}{c|}{VIS} &  \multicolumn{2}{c|}{VPS} & \multicolumn{1}{c|}{VOS} & \!RefVOS \\
\hline
\multirow{2}{*}{\!\!Stage 3} & \multirow{2}{*}{ Tracker} & {\!YT21}  & {\!OVIS} & \multicolumn{2}{c|}{ VIPSeg} & YT18  & RefYT \ \\
     & & mAP & mAP & \!VPQ & \!STQ & $G^{th}$ & J\&F \\
\hline
\crossmark & Similarity  & 50.7 & 15.0 & 42.0 & 38.1 & 60.8 & \\
\crossmark & P$\rightarrow$Q   & 52.7 & 21.7 & 38.6 & 45.8 & 67.4 & \\
% $\checkmark$ & Learnable & MinVIS  & \\
$\checkmark$ & P$\rightarrow$Q   & 54.7 & 23.6 &    &      & 69.2 & \\ % 54.3 & 23.4 \\
\Xhline{0.8pt}
\end{tabular}
}
\vspace{-2mm}
\caption{\small Ablation studies on the types of trackers (We use dev set for VIS tasks). The trackers of 'Similarity' and 'P$\rightarrow$Q' indicate the embedding similarity matching and our proposed transformation from any entity to a prompt-guided target, respectively.
} \label{tab:abl_details}
\vspace{-2mm}
\end{table}

==> tables/sota_img_strong_bb.tex <==
\begin{table*}[!t]
\centering
{\small 
\begin{tabular}{p{0.1\linewidth}p{0.075\linewidth}<{\centering}p{0.05\linewidth}<{\centering}|p{0.025\linewidth}<{\centering}p{0.025\linewidth}<{\centering}p{0.035\linewidth}<{\centering}|p{0.08\linewidth}<{\centering}|p{0.025\linewidth}<{\centering}p{0.025\linewidth}<{\centering}p{0.035\linewidth}<{\centering}}
\Xhline{0.8pt}
\rowcolor{LightCyan}
\multicolumn{3}{l|}{\small Image Tasks} & \multicolumn{3}{c|}{Generic seg.}  & \multicolumn{1}{c|}{REC} & \multicolumn{3}{c|}{Zero-shot seg.}  \\
\hline\hline
 \multirow{2}{*}{\small Method} & \multirow{2}{*}{Backbone } & One-& \multicolumn{3}{c|}{\small COCO}  & RefCOCO & \multicolumn{3}{c}{\small Ade20k} \ \\
  & & Model & PQ & mAP & mIoU & J\&F & PQ & mAP & mIoU\ \\
\hline
\multicolumn{3}{l}{\color{blue} \it Specific models} \\
\hline
Mask2Former & Swin-L & \crossmark \\
X-Decoder   & Swin-L & \crossmark \\
\hline 
\multicolumn{3}{l}{\color{blue} \it Unified models} \\
\hline 
SEEM      & & $\checkmark$ \\
UNINEXT   & & $\checkmark$ \\
Sem-SAM   & & $\checkmark$ \\
UniVS (our) & Swin-B & $\checkmark$ \\
UniVS (our) & Swin-L & $\checkmark$ \\
\Xhline{0.8pt}
\end{tabular}
}
\vspace{-2mm}
\caption{\small Overall comparison on stronger backbones. 
} \label{tab:sota_swin}
\vspace{-2mm}
\end{table*}

==> tables/sota_r50_img.tex <==
\begin{table*}[!t]
\centering
{\footnotesize
\begin{tabular}{p{0.09\linewidth}p{0.09\linewidth}<{\centering}p{0.05\linewidth}<{\centering}p{0.055\linewidth}<{\centering}|p{0.02\linewidth}<{\centering}p{0.025\linewidth}<{\centering}p{0.03\linewidth}<{\centering}|p{0.08\linewidth}<{\centering}|p{0.05\linewidth}<{\centering}p{0.055\linewidth}<{\centering}p{0.055\linewidth}<{\centering}|p{0.085\linewidth}<{\centering}}
\Xhline{0.8pt}
\rowcolor{LightCyan}
\multicolumn{4}{c|}{ Image Tasks} & \multicolumn{3}{c|}{Generic seg.}  & \multicolumn{1}{c|}{REC} & \multicolumn{3}{c|}{Interactive seg.} & Eentity seg. \\
\hline\hline
\multirow{2}{*}{ Method} & \multirow{2}{*}{ Backbone} & Joint & \multirow{2}{*}{\!Universal} & \multicolumn{3}{c|}{ COCO}  & RefCOCOg & \multicolumn{3}{c|}{ PascalVOC} & ES \ \\
 & & Training &   & \!mAP &  PQ & \!\!mIoU  & cIoU & {\scriptsize \!\!5-NoC85} & {\scriptsize \!\!10-NoC85} & {\scriptsize \!\!20-NoC85} & OWTA$_\text{all}$ \\
 \hline
Mask2Former & R50 & \crossmark & \crossmark & 41.7 & 51.9 & 61.7 & -    & - & -    & - & -\\
UNINEXT     & R50 & $\checkmark$ & \crossmark & 44.9 & -    & -  & 70.2 & -    & - & - & - \\
UniVS       & R50 & $\checkmark$ & $\checkmark$ & 42.2 & 47.8 & 59.8   \\

\hline
Mask2Former & Swin-T & \crossmark & \crossmark & 43.3 & 53.2 & 63.2 & -    & - & -    & - & - \\
X-Decoder   & Swin-T & \crossmark & \crossmark & 41.3 & 52.6 & 62.4 & 61.9 & - & -    & - & - \\
SEEM        & Swin-T & $\checkmark$ & $\checkmark$ & 39.7 & 50.8 & 62.2 & 60.9 & 1.72 & 2.30 & 3.37 & * \\
DINOv       & Swin-T & $\checkmark$ & $\checkmark$ & 41.5 & 49.0 & 57.0 &  \\
UniVS       & Swin-T & $\checkmark$ & $\checkmark$ & 42.4 & 49.2 & 62.3 & \\
\hline
Mask2Former & Swin-B & \crossmark & \crossmark & 45.2 & 55.1 & 65.1 & -    & - & -    & - & - \\
X-Decoder   & Swin-B & \crossmark & \crossmark & 45.8 & 56.2 & 66.0 & 64.5 & - & -    & - & - \\
SEEM        & Swin-B & $\checkmark$ & $\checkmark$ & 46.4 & 56.1 & 66.3 & 65.0 & 1.56 & 2.04 & 2.93 & * \\
UniVS       & Swin-B & $\checkmark$ & $\checkmark$ & 46.4 & 54.3 & 66.1  \\
\hline
Mask2Former & Swin-L & \crossmark & \crossmark & 48.6 & 57.8 & 67.4 & -    & - & -    & - & - \\
X-Decoder   & Swin-L & \crossmark & \crossmark & 46.7 & 56.9 & 67.3 & 64.6 & - & -    & - & - \\
UNINEXT     & ConvNextL  & $\checkmark$ & \crossmark & 49.6 & -    & -  & 73.4 & -    & - & -  & - \\
% UNINEXT     & Vit-H      & $\checkmark$ & \crossmark & 51.8 & -    & -  & 74.7 & -    & - & - & - \\
SEEM        & Swin-L     & $\checkmark$ & $\checkmark$   & 47.7 & 57.5 & 67.6 & 65.6 & 1.51 & 1.95 & 2.77  & * \\
DINOv       & Swin-L     & $\checkmark$ & $\checkmark$   & 50.4 & 57.7 & 66.7 &  \\
UniVS       & Swin-L     & $\checkmark$ & $\checkmark$   & 48.0 & 55.4 & 67.1 & \\
\Xhline{0.8pt}
\end{tabular}
}
\vspace{-2mm}
\caption{ Overall comparison on image datasets. `-' and `*' indicate the model lack capability and no reported number for the task, respectively.
} \label{tab:sota_r50}
\vspace{-2mm}
\end{table*}

==> tables/sota_r50_vid.tex <==
\begin{table*}[!t]
\centering
{\footnotesize
\begin{tabular}{p{0.13\linewidth}p{0.0325\linewidth}<{\centering}p{0.05\linewidth}<{\centering}|p{0.03\linewidth}<{\centering}p{0.025\linewidth}<{\centering}p{0.035\linewidth}<{\centering}|p{0.03\linewidth}<{\centering}p{0.037\linewidth}<{\centering}|p{0.028\linewidth}<{\centering}p{0.028\linewidth}<{\centering}|p{0.03\linewidth}<{\centering}p{0.035\linewidth}<{\centering}|p{0.052\linewidth}<{\centering}p{0.035\linewidth}<{\centering}|p{0.052\linewidth}<{\centering}}
\Xhline{0.8pt}
\rowcolor{LightCyan}
\multicolumn{3}{c|}{Video Tasks} & \multicolumn{3}{c|}{VIS} &  \multicolumn{2}{c|}{VSS} &  \multicolumn{2}{c|}{VPS} & \multicolumn{2}{c|}{VOS} & \multicolumn{2}{c|}{RefVOS} & PVOS \\
\hline
 \multirow{2}{*}{\!\!Method}& \multirow{2}{*}{ \!\!\!\!Unified} & \multirow{2}{*}{ \!\!\!\!Universal} & {\!YT19} & { YT21}  & { OVIS} &  \multicolumn{2}{c|}{ VSPW} & \multicolumn{2}{c|}{ VIPSeg} &{ \!DAVIS} &{ YT18\ } & \!\!RefDAVIS & \!\!RefYT & \!\!VIPOSeg \ \\
  & & & mAP & mAP & mAP & mIoU & \!mVC$_8$ & \!VPQ & \!STQ & $G^{th}$ & $G^{th}$ & J\&F & J\&F & $G^{th\&sf}$ \\
\hline
%\!\!IDOL\cite{IDOL}         & \crossmark & \crossmark & 49.5 & 43.9  & 30.2 & - & - & - & - & - & - & -& - & - \\
\!\!MinVIS\cite{huang2022minvis}       & \crossmark & \crossmark & 47.4 & 44.2  & 25.0 & -  & - & - & - & - & - & -& - & - \\
\!\!MDQE\cite{li2023mdqe}         & \crossmark & \crossmark & *    & 44.5  & 29.2 & - & - & - & - & - & -& - & - & - \\
\!\!GenVIS-off\cite{GenVIS}   & \crossmark & \crossmark &  {51.3} &  {46.3}  &  {34.5} & - & - & - & - & - & - & - & - & - \\
\!\!TCB+ResNet101\cite{vspw}      & \crossmark & \crossmark & - & - & - &  {37.8} &  {87.8}  & - & - & - & - & - & - & - \\
\!\!\!ClipPanoFCN\cite{vipseg} & \crossmark & \crossmark & - & - & - & - & - &  {22.9} &  {31.5} & - & - & -  & - & - \\
\!\!XMem\cite{xmem}         & \crossmark & \crossmark & - & - & - & - & - & - & - &  {86.2} & 85.7  & - & - & - \\ % mose: 56.3
\!\!DeAOT\cite{yang2022deaot}        & \crossmark & \crossmark & - & - & - & - & - & - & - & 85.2 &  {86.0} & - & - & - \\ % mose: 59.0
\!\!ReferFormer\cite{referformer}  & \crossmark & \crossmark & - & - & - & - & - & - & - & - & -  & 58.5 & 55.6 & -\\
\!\!OnlineRefer\cite{wu2023onlinerefer}  & \crossmark & \crossmark & - & - & - & - & - & - & - & - & -  & 59.3 & 57.3 & -\\
\!\!SgMg+SwinT\cite{Miao_2023_ICCV_sgmg}   & \crossmark & \crossmark & - & - & - & - & - & - & - & - & -  &  {61.9} &  {62.0} & -\\
\!\!PAOT\cite{xu2023viposeg}         & \crossmark & \crossmark & - & - & - & - & - & - & - & - & -  & - & - &   {75.4} \\
\hline 
% \hline
\!\!VideoK-Net\cite{videoknet}  & $\checkmark$ & \crossmark & 40.5  &  * & * & * & 26.1 & 33.1 & - & - & - & - & - \\ % 21
\!\!Video-kMax\cite{videokmax}  & $\checkmark$ & \crossmark & * & * & * &  {44.3} & 86.0 & 38.2 & 39.9 & - & - & - & - & - \\ % 23
\!\!Tube-Link\cite{tubelink}   & $\checkmark$ & \crossmark &  {52.8} &  {47.9} & 29.5 & 42.3 &  {86.8} & 39.2 & 39.5 & - & - & - & - & - \\ % iccv23
% \!\!DVIS-on\cite{dvis}      & $\checkmark$ & \crossmark & 51.2 & 46.4 & 30.2 & * & * & \multirow{2}{*}{ {43.2}} & \multirow{2}{*}{ {42.8}} & - & - & - & - & - & - \\ % iccv23
\!\!DVIS-off\cite{dvis}     & $\checkmark$ & \crossmark & 52.6 & 47.4 &  {33.8} & * & * & 43.2 & 42.8 & - & - & - & - & - \\ % iccv23
\!\!UniRef\cite{Wu_2023_ICCV_uniref}       & $\checkmark$ & \crossmark & - & - & - & - & - & - & - & * &  {81.4} & 63.5 & 60.6 & * \\  % iccv23
\hline 
\!\!TarVIS\cite{tarvis}       & $\checkmark$ & \crossmark &  * & 48.3 & 31.1 & * & * &  33.5 & 43.1 &  {82.6} & * & - & - & - \\  % cvpr23
\!\!UNINEXT\cite{uninext}      & $\checkmark$ & \crossmark &  {53.0} & *  &  {34.0} & - & -  & - & - & 74.5 & 77.0 &  {63.9} &  {61.2} & - \\ % cvpr23
\!\!UniVS       & $\checkmark$ & $\checkmark$   & 46.9 & 46.6  & 29.9 &  {48.2} &  {88.5} & 38.6  & 45.8 & 68.0 & 69.2 & 57.5 & 55.4 & * \\ % mose: & 45.5
\!\!UniVS+SwinT  & $\checkmark$ & $\checkmark$   & 52.4 &  {51.6}  & 33.0 & 51.3 & 89.4 &  {38.9} &  {51.7} & 69.4 & 70.3 & 58.5 & 56.2 & * \\ % mose: & 46.3
% \!\!UniVS+SwinB   & $\checkmark$ & $\checkmark$ & 57.8 & 56.5 & 38.4 & 59.4 & 90.4 &  &  & & &   \\
% \!\!UniVS+SwinL   & $\checkmark$ & $\checkmark$ & 60.0 & 57.7 & 40.4 & 59.8  & 92.3  & 49.3 & 58.2  &  \\
\Xhline{0.8pt}
\end{tabular}
}
\vspace{-3mm}
\caption{\small Overall quantitative performance comparison on ResNet50/101 or SwinT backbone, where the default is ResNet50. `-' or `*' indicate the model lack capability or no reported number for the task, respectively. GenVIS-off\cite{GenVIS}, DVIS-off\cite{dvis}, XMem\cite{xmem} and DeAOT\cite{yang2022deaot} incorporate long-term propagation modules and fine-tune them with multiple clips during training to achieve higher performance.
} \label{tab:sota_r50}
\vspace{-2mm}
\end{table*}

==> tables/sota_vid_strong_bb.tex <==
\begin{table*}[!t]
\centering
{\footnotesize
\begin{tabular}{p{0.11\linewidth}p{0.075\linewidth}<{\centering}p{0.03\linewidth}<{\centering}p{0.048\linewidth}<{\centering}|p{0.025\linewidth}<{\centering}p{0.023\linewidth}<{\centering}p{0.03\linewidth}<{\centering}|p{0.02\linewidth}<{\centering}p{0.028\linewidth}<{\centering}|p{0.022\linewidth}<{\centering}p{0.022\linewidth}<{\centering}|p{0.025\linewidth}<{\centering}p{0.035\linewidth}<{\centering}|p{0.032\linewidth}<{\centering}p{0.032\linewidth}<{\centering}|p{0.05\linewidth}<{\centering}}
\Xhline{0.8pt}
\rowcolor{LightCyan}
\multicolumn{4}{c|}{Video Tasks} & \multicolumn{3}{c|}{VIS} &  \multicolumn{2}{c|}{VSS} &  \multicolumn{2}{c|}{VPS} & \multicolumn{2}{c|}{VOS} & \multicolumn{2}{c|}{RefVOS} & PVOS \ \\
\hline\hline
 \multirow{2}{*}{\!\!Method} & \multirow{2}{*}{Backbone} & \multirow{2}{*}{ \!\!\!\!Unified} & \multirow{2}{*}{ \!\!\!\!Universal} & { \!YT19} & { YT21}  & { \!OVIS} &  \multicolumn{2}{c|}{ VSPW} & \multicolumn{2}{c|}{ VIPSeg} & \!\!DAVIS & { \!YT18 }   & \!\!DAVIS & \!\!\!RefYT & \!\!\!VIPOSeg\ \\
  & & & & mAP & mAP &  mAP & \!\!mIoU & \!\!\!mVC$_8$ & \!VPQ & \!STQ & $G^{th}$ & $G^{th}$ & J\&F & J\&F &$G^{th\&sf}$ \\
\hline
\!\!IDOL\cite{IDOL}         &  Swin-L & \crossmark & \crossmark & 49.5 & 43.9 & 42.6 & - & - & - & - & - & -  & -& - & -\\
\!\!MinVIS\cite{huang2022minvis}       &  Swin-L & \crossmark & \crossmark & -    & 55.3 & 41.6 & - & - & - & - & - & -  & -& -  & -\\ % nips22
\!\!GenVIS-off\cite{GenVIS}   &  Swin-L & \crossmark & \crossmark & 63.8 & 60.1 & 45.4 & - & - & - & - & - & -  & -& -  & -\\ % cvpr23
\!\!CFFM\cite{CFFM_vss}         & MiT-B5  & \crossmark & \crossmark & - & - & - & 49.3 & 90.8  & - & - & - & -   & - & - & -\\
\!\!DeAOT\cite{yang2022deaot} & Swin-B  & \crossmark & \crossmark & - & - & - & - & - & - & - & 86.2 & 86.2  & - & - & - \\ % nips22
% \!\!JointFormer & ConvMAE-B & \crossmark & \crossmark & - & - & - & - & - & - & - & 89.7 & 87.0 & * & - & - & - \\ % 25-Aug-23, ConvMAE-Base is a strong backbone
\!\!ReferFormer\cite{referformer}  & Swin-L  & \crossmark & \crossmark & - & - & - & - & - & - & - & - & - & 60.5 & 62.4 & - \\  % 2022
\!\!OnlineRefer\cite{wu2023onlinerefer}  & Swin-L & \crossmark & \crossmark & - & - & - & - & - & - & - & - & -  & 64.8 & 63.0 & - \\ % iccv23
\!\!SgMg\cite{Miao_2023_ICCV_sgmg}        & SwinB   & \crossmark & \crossmark & - & - & - & - & - & - & - & - & -  & 63.3 & 65.7 & -\\  % iccv23
\!\!PAOT\cite{xu2023viposeg}        & SwinB   & \crossmark & \crossmark & - & - & - & - & - & - & - & - & -  & - & - &  75.3 \\  % 25-Jun-23
\hline 
\multicolumn{8}{l}{\color{blue} \it Unified models trained individually on each dataset} \\
\hline
\!\!TubeFormer\cite{tubeformer}   &  A-R50$\times$64 & $\checkmark$ & \crossmark & 47.5 & 41.2 & * & 63.2 & 92.1 & *  & * & - & - & - & -& - \\
\!\!VideoK-Net+\cite{videoknet} & Swin-B & $\checkmark$ & \crossmark & 51.4 & * & * & * & * & 39.8 & 46.3 & - & - & - & - & - \\
\!\!Video-kMax\cite{videokmax}   & ConvNeXtL & $\checkmark$ & \crossmark & * & * & * & 63.6 & 91.8 & 51.9 & 51.7 &  - & - & -  & -& - \\
\!\!Tube-Link\cite{tubelink}    & Swin-L & $\checkmark$ & \crossmark & 64.6 & 58.4 & * & 59.7 & 90.3 & * & * & - & - & - & - & - \\  % iccv23
% \!\!DVIS-on\cite{dvis}      & Swin-L & $\checkmark$ & \crossmark & 63.9 & 58.7 & 47.1 & * & * & \multirow{2}{*}{57.6} & \multirow{2}{*}{55.3} & - & -  & - & -& - \\ % iccv23
\!\!DVIS-off\cite{dvis}     & Swin-L & $\checkmark$ & \crossmark & 64.9 & 60.1 & 49.9 & * & * & 57.6 & 55.3  & - & - & - & -& - \\ % iccv23
\hline
\multicolumn{8}{l}{\color{blue} \it Unified models trained jointly on multiple tasks} \\
\hline
\!\!UniRef\cite{Wu_2023_ICCV_uniref}       & Swin-L   & $\checkmark$ & \crossmark & - & - & - & - & - & - & - & * & 82.6 &  66.3 & 67.4 & * \\  % iccv23
\!\!TarVIS\cite{tarvis}       & Swin-L    & $\checkmark$ & \crossmark &  *   & 60.2 & 43.2 & * & * & 48.0 & 52.9 & 85.2 & * & - & - & -  \\
\!\!UNINEXT\cite{uninext}      & ConvNeXtL & $\checkmark$ & \crossmark & 64.3 & *    & 41.1 & - & - & - & - & 77.2 & 78.1 & 66.7 & 66.2 & -\\ % cvpr23
\!\!\textcolor{gray}{UNINEXT}\cite{uninext}      & \textcolor{gray}{ViT-H}    & \textcolor{gray}{ $\checkmark$} & \textcolor{gray}{\crossmark} & \textcolor{gray}{66.9} & \textcolor{gray}{ *}    & \textcolor{gray}{49.0} & \textcolor{gray}{-} & \textcolor{gray}{-} & \textcolor{gray}{-} & \textcolor{gray}{-} & \textcolor{gray}{81.8} &\textcolor{gray}{78.6} & \textcolor{gray}{72.5} & \textcolor{gray}{70.1} & \textcolor{gray}{-}\\ % cvpr23
\!\!UniVS        & Swin-B   & $\checkmark$ & $\checkmark$ & 57.8 & 56.5 & 39.0 & 59.4 & 90.4 & 46.7 & 56.1  & 70.8 & 70.9 & 58.6 & 57.4 & 68.2 \\
\!\!UniVS        & Swin-L   & $\checkmark$ & $\checkmark$ &  60.0 & 57.9 & 41.7 & 59.8  & \textbf{92.3}  & 49.3 & \textbf{58.2}  & 71.1 & 71.5 & 59.4 & 58.0 & 68.6  \\
\Xhline{0.8pt}
\end{tabular}
}
\vspace{-2mm}
\caption{\small Overall quantitative performance comparison on stronger backbones. `-' and `*' indicate the model lack capability and no reported number for the task, respectively. GenVIS-off\cite{GenVIS}, DVIS-off\cite{dvis}, Xmem\cite{xmem} and DeAOT\cite{yang2022deaot} incorporate long-term information propagation modules and utilize multiple video clips to fine-tune these modules during training, obtaining higher performance.
} \label{tab:sota_strong_vid}
\end{table*}
